Computational Complexity of Interactive Behaviors

The theory of computational complexity focuses on functions and, hence, studies programs whose interactive behavior is reduced to a simple question/answer pattern. We propose a broader theory whose ultimate goal is expressing and analyzing the intrinsic difficulty of fully general interactive behaviors. To this extent, we use standard tools from concurrency theory, including labelled transition systems (formalizing behaviors) and their asynchronous extension (providing causality information). Behaviors are implemented by means of a multiprocessor machine executing CCS-like processes. The resulting theory is shown to be consistent with the classical definitions: when we restrict to functional behaviors (i.e., question/answer patterns), we recover several standard computational complexity classes.

==> Ev.tex <==
\dm{I don't give the exact definitions, just a sketch of what I need in \refsect{Compl}. Anything equivalent will do.}
\dv{I stay informal too for the moment}
In order to define the complexity measures, we need to fomalise concurrency and causality of events. There are several models in the literature that could be used. In this presentation
we will use the model of Mazurkiewicz traces~\cite{Maz86,WN95}. In order to formally define a notion of events some technicalities need to be added to the semantics of the
process machine. Let $\tags$ be the set of nonempty finite strings over $\{l,r\}$. In a configuration of a process machine we assume every two occurences of  process states
have incomparable tags from $\tags$. If $t$ is a tag of a parallel composition, the two spawned process states have tags $tl$ and $tr$. It is easy to see that this maintains the invariant.
Transitions are now tagged with the tag of the process state that they correspond to.

We define now and independence relation on tagged transitions. All tau transitions could be identified, except for send and receive.
The independence relation is defined as follows. Tau, input and output transitions on different tags are independent.
Send and receive transitions are independent from any tau, input, output transition on a different tag.
Send and receive transitions are independent from any send and receive transitions on a different tag and on a different queue.

In particular two send/receive transitions on the same queue are never independent. This amount to forbid concurrent access to a queue, even
when this could be safe. We could consider queues with concurrent access too. In this case send and receive on different tags would be always independent except when one is an send on an empty queue and
the other is an receive on the same queue. But this complicates the details, as states should be considered in defining the independence relation.

\begin{definition}[Run]
	A \emph{run} is a finite, possibly empty sequence of consecutive tagged transitions $\runone=\cfgone_0\mtrans{\acone_1}\cdots\mtrans{\acone_n}\cfgone_n$, where $\cfgone_0,\ldots,\cfgone_n$ are configurations.
\end{definition}

 We use $\trone$ to range over transitions, and we denote concatenation of runs bu juxtaposition. 

Following the theory of Mazurkiewicz traces,
% After the lts of a process is endowed with an ``independence structure'' (\ie, it becomes a lts with independence), 
an equivalence $\eqrun$ between runs is defined. Then, a preorder between runs may be defined by $\runone\prerun\runtwo$ iff $\runtwo\sim\runone\runone'$ for some run $\runone'$.
\begin{definition}[Essential run, event, causal order]
\dv{If you prefer I could follow more closely the approach of \cite{WN95}}
	In the following, we fix a closed process and consider the set of Mazurkiewicz traces it generates. A run is \emph{essential} if it is of the form $\runone\trone$ and, whenever $\runtwo\eqrun\runone\trone$, we have $\runtwo=\runone'\trone$ and $\runone'\eqrun\runone$.

	An \emph{event} $\evone$ is a $\eqrun$-equivalence class of essential runs. Given an event $\evone$, all runs $\runone\in\evone$ end with the same transition $\cfgone\mtrans{\acone}\cfgone'$; we define the \emph{action} of $\evone$ to be $\evlab{\evone}=\acone$, and we say that $\evone$ is an input, output, or internal event according to whether $\acone$ is an input, output, or internal action.

	The \emph{causal order} between events, denoted by $\leq$, is defined as the quotient of $\prerun$ modulo $\eqrun$.
\end{definition}


==> FnServ.tex <==
\newcommand{\subst}[2]{%
  % substitute #1 for #2
  \{{}^{#1}\!/_{#2}\}%
}
\begin{example}[Function servers]
  \label{ex:functionServer}
  Let $\procone_f$ be a process that implements some function $f \colon \Words \to \Words$, 
  i.e.\ $\labsem\procone_f$ is a functional behavior. 
  Roughly $\procone_f$ will calculate the function  $f$ only once. 
  If one wants in fact the function $f$ to behave ``as usual''
  in programming languages, the behavior one actually wants 
  is given by the zeroary process identifier $\pvarone_f$ with $\pvarone_f = \para{\procone_f}{\pvarone_f}$, 
  which we shall call the function server of $f$. 

  Now consider, the ``more lazy'' variation of this function server, 
  namely the process identifier $\pvartwo_f$ with 
  \begin{displaymath}
    \pvartwo_f = \inpc{\ichan}{\evarone}
    \left( 
      \para{
        \outc{\mathtt{1}}{\evarone}\proczero
      }
      {
        \para{
          \procone_f \subst{\mathtt{1}}{\ichan}\subst{\mathtt{0}}{\ochan}
        }
        {
          \inpc{\mathtt{0}}{\evartwo}\outc{\ochan}{\evartwo}\pvartwo_f
        }
      }
    \right)
  \end{displaymath}
  where $\procone_f \subst{\mathtt{1}}{\ichan}\subst{\mathtt{0}}{\ochan}$ 
  is $\procone_f$ with all relevant occurrences of $\ichan$ and $\ochan$ 
  replaced by $\mathtt{1}$ and $\mathtt{0}$ respectively
  (and we assume w.l.o.g. that $\mathtt{1}$ and $\mathtt{0}$ are not used in $\procone_f$). 
  This lazy function server only has one active instance of $\procone_f$ at each point in time. 
\end{example}
\tbh{%
  Now the exercise is to calculate the complexity of $\pvartwo_f$.
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> Streams.tex <==
Continous and computable function from streams to streams (actually from any string to any string (finite and infinite))

First complexity: as function from finite strings to finite strings ("eventually strictly" monotonic)
Alternative complexity: ask for an extra bit when needed (interactive computation). This is more the point of view as a function from streams to streams (or as real number computation with arbitrary precision)

Damiano's trick for ensuring you just ask for ONE bit of input.


==> StructuredIntro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% opening paragraph, catching attention [optional]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Highly interactive computing devices have become an essential part 
of day to day live, be it in the form of mediators of human actions, 
controllers of life support systems, or embedded systems in vehicles on earth and in outer space. 
In particular, computers are not restricted anymore to answering yes/no questions
or number crunching functions without affecting the real world.  
To study this phenomenon of \emph{interactive} computation\verb+citeWegener+, 
theoretical computer scientists have developed several 
formalisms and methodologies, such as process calculi and algebras. 
However, computational complexity has not much to say about this area, yet, 
and is of no help if we ask ``How can we measure the efficiency of an interactive system?'' 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     motivation & problem statement
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We take it that computational complexity theory is meant 
to study the performance of programs, or more precisely the intrinsic difficulty to solve a 
given problem (using a fixed programming framework).
So we ask ``What is the intrinsic difficulty of interactive computing tasks? What characterizes the class of interactive tasks
that can be accomplished efficiently by processes?'' 
Note that we cannot just apply existing methods of computational complexity theory 
to interactive systems: for instance, traditionally, 
the amount of resources consumed by programs is measured
by certain fixed or parametric bounds that do not take into account 
\emph{arbitrary} interaction of a program with its environment. 
And even if interaction is taken into account in one way or another (e.g., in interactive
proofs~\cite{}), it is often seen as yet another way to compute functions (i.e., the class $\mathsf{IP}$ 
is a class of functions). \tbh{What about online algorithms?}
Complexity analysis of online and streaming algorithms, on the other hand, 
only deal with a specific interaction pattern. We set out to revise computational 
complexity to obtain concepts and methods for the  classification of the efficiency
of genuinely interactive behaviors. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     related work: standing on the shoulders of giants
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As behaviors are usually defined using labelled transition systems (\textsc{lts}s),
the first idea is to use a process calculus, such as Milner's CCS, 
as specification language for processes.
Though process calculi are the model of choice to specify behaviours, 
they do not incorporate any notion of  ``resources'' and thus are too abstract for our purpose; 
moreover, traditionally, there is no notion of concurrency in process calculi 
and thus the potential of parallel computation is not represented. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     contribution and results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tbh{This paragraph needs most revision I think.}
To address the last two problems, we introduce first a \emph{process machine} 
that is inspired by process calculi but is more concrete and comes with natural notion of resource;
moroever, we give our process machine a  \emph{truly concurrent} semantics in terms of
asynchronous transition systems \textsc{alts}~\cite{WN95}.
 The process machine gives rise to concrete examples of what we call 
\emph{weighted asynchronous labeled transition systems} \textsc{walts}s, which are 
\textsc{alts} with a suitable cost model that allows to measure the time and space 
cost of events in interactive computations. 
Moreover, \emph{behaviors} are introduced as an extensional concept analogous 
to \emph{functions} in non-interactive computation: they are equivalent classes 
of processes with respect to a suitable notion of bisimulation.
Thus, as we shall argue, the process machines provides at the same 
time a cost model and a programming language for behaviours.
As a sanity check, we show that our definitions of cost and complexity coincide with 
the standard ones when restricted to the so called \emph{functional} behaviours, i.e.,  
behaviours that correspond to the non-interactive computations of Turing machines.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     structure/overview of the paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> Traces.tex <==
The following is taken from~\cite{WN95}. 

\begin{definition}
  \label{def:MazTraceLang}
  A \emph{Mazurkiewicz trace language}
  consists of $(M,L,I)$ where
  $L$ is a set, 
  $I \subseteq L \times L$ is a symmetric, irreflexive relation 
  called the \emph{independence} relation, 
  and $M$ is a nonempty subset of strings $L^*$ 
   that is
  \begin{itemize}
  \item
    \emph{prefix closed:} $sa \in M \Rightarrow s \in M$ 
    for all $s \in L^*$, $a \in L$,
  \item
    \emph{$I$-closed:} $sabt \in M \land a\mathrel{I}b \Rightarrow sabat \in M$
    for all $s,t \in L^*$, $a,b \in L$,
  \item 
    \emph{coherent:} $sa \in M \land sb \in M \land a \mathrel{I} b \Rightarrow sab \in M$
    for all $s \in L^*$, $a,b \in L$. 
  \end{itemize}
\end{definition}

\newcommand{\tc}[1]{%
  % the equivalence class of a string / a Mazurkiewicz trace
  \{#1\}_{\eqsim}%
}
\begin{definition}
  Let $(M,L,I)$ be  a trace language. 
  For $s,t \in M$ define $\eqsim$ to be the smallest equivalence relation such that 
  \begin{displaymath}
    sabt \eqsim sbat \text{ if } a\mathrel{I}b
  \end{displaymath}
  for $sabt, sbat \in M$. 
  Call an equivalence class $\tc{s}$, 
  for $s \in M$, a \emph{trace}. 
  For $s,t \in M$ define 
  \begin{displaymath}
    s \lesssim t \iff \exists u \ldotp su \eqsim t. 
  \end{displaymath}
\end{definition}

\paragraph{From trace languages to event structures}
\label{par:traceToEvStr}


\newcommand{\ec}{%
  % event class of a string
  % 
}
\begin{definition}
  The relation $\sim$ is the smallest equivalence relation on nonempty strings such that
  \begin{align*}
    sa &\sim sba &&\text{ if } b \mathrel{I} a, \text{ and}\\
    sa &\sim ta  &&\text{ if } s \eqsim t 
  \end{align*}
  for $sa, sba, ta \in M$. 
\end{definition}


\newcommand{\evc}[1]{%
  % event class of a string
  \{#1\}_{\sim}%
}

\newcommand{\ev}{\mathit{ev}}
\begin{definition}[Events of a string]
  \label{def:eventsOfAstring}
  Let $s \in M$. 
  Define the events of $s$ to be
  \begin{displaymath}
    \ev(s) = \{ \evc{u} \mid u \text{ is a nonempty prefix of } s \}
  \end{displaymath}
\end{definition}

\newcommand{\tle}{%
  \mathit{tle}%
}
\renewcommand{\sharp}{%
  \mathrel{\#}%
}
\begin{definition}[Event structure of a trace language]
  \label{def:EvStrFromTraceLang}
  Let $T = (M,L,I)$ be a trace language. 
  Define
  \begin{displaymath}
    \tle(M,L,I) = (e, \leq, \sharp)
  \end{displaymath}
  where
  \begin{itemize}
  \item 
    $E$ is the set of events of $(M,L,I)$, 
  \item 
    $\leq$ is a relation between events $e, e'$ 
    given by $e \leq e'$
    iff $e \in \ev(s)$
    where $sa$ is a minimum representative of $e'$, 
    and 
  \item 
    the relation $e \sharp e'$ holds between events iff
    \begin{displaymath}
      \exists e_0, e_0'\ldotp e_0 \sharp_0 e_0' \land e_0 \leq e \land e_0' \leq e'
    \end{displaymath}
    where, by definition, 
    \begin{displaymath}
      e_0 \sharp_0 e_0' \text{ iff } \exists v,a,b\ldotp va \in e_0 \land vb \in e_0' \land \neg (a \mathrel{I} b) \land  a\neq b.
    \end{displaymath}
  \end{itemize}
  Furthermore, define $\lambda_T \colon E \to L$ by taking $\lambda_T(\evc{sa}) = a$. 
  (From the definition of $\sim$, it follows that the function $\lambda_T$ is well-defined.)
\end{definition}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

